Intense Laser-Driven Phenomena In Weyl Semimetals

Condensed-matter provides attractive platforms to realize exotic particles, originally proposed in high-energy physics. Weyl semimetal (WSM) is a material in which low-energy collective excitations are governed by massless Weyl fermions, which appear in pairs of opposite chirality and are topologically protected. Thus, the discovery of topological materials such as WSM has heralded a new era in contemporary physics. Moreover, these materials offer exciting opportunities in next-generation signal processing and optoelectronics. This thesis explores different facets of the intense laser-driven phenomena in WSM for applications in emerging lightwave-driven Petahertz electronics and quantum technologies.

==> HeadTail/certi.tex <==
\newpage
\thispagestyle{empty}
 \vspace*{2cm}
\begin{center}
\textbf{\Large\underline {Approval Sheet}}
\end{center}
\vspace{1cm}
This thesis entitled \textbf{High-harmonic Spectroscopy of Two-dimensional Materials} by \textbf{Mrudul M. S.} (Roll No. 164120007) is approved for the degree of Doctor of Philosophy in Physics.

\begin{flushright}
\textbf{Examiners}\\
\-------------------------\\
\-------------------------\\
\-------------------------\\



\textbf{Supervisor}\\
Dr. Gopal Dixit

\textbf{Chairman}\\
\-------------------------\\


\end{flushright}

\begin{flushleft}
Date :\\
Place :
\end{flushleft}


